A Color Elastica Model for Vector-Valued Image Regularization

Models related to the Euler's elastica energy have proven to be useful for many applications including image processing. Extending elastica models to color images and multi-channel data is a challenging task, as stable and consistent numerical solvers for these geometric models often involve high order derivatives. Like the single channel Euler's elastica model and the total variation (TV) models, geometric measures that involve high order derivatives could help when considering image formation models that minimize elastic properties. In the past, the Polyakov action from high energy physics has been successfully applied to color image processing. Here, we introduce an addition to the Polyakov action for color images that minimizes the color manifold curvature. The color image curvature is computed by applying of the Laplace-Beltrami operator to the color image channels. When reduced to gray-scale images, while selecting appropriate scaling between space and color, the proposed model minimizes the Euler's elastica operating on the image level sets. Finding a minimizer for the proposed nonlinear geometric model is a challenge we address in this paper. Specifically, we present an operator-splitting method to minimize the proposed functional. The non-linearity is decoupled by introducing three vector-valued and matrix-valued variables. The problem is then converted into solving for the steady state of an associated initial-value problem. The initial-value problem is time-split into three fractional steps, such that each sub-problem has a closed form solution, or can be solved by fast algorithms. The efficiency and robustness of the proposed method are demonstrated by systematic numerical experiments.

==> tmp_main_abstract.tex <==
		\begin{abstract}
			Models related to the Euler's elastica energy have proven to be useful for many applications including image processing. % and high energy physics.
			Extending elastica models to color images and multi-channel data is a challenging task, as stable and consistent numerical solvers for these geometric models often involve high order derivatives.
			%The question of what could be considered as  appropriate image regularization is important  in image processing.
			Like the single channel Euler's elastica model and the total variation (TV) models, geometric measures that involve high order derivatives could help when considering image formation models that minimize elastic properties.
			% \rk{unclear - "minimal elastica properties"?}
			In the past, the Polyakov action from high energy physics has been successfully applied to color image processing.
			Here, we introduce an addition to the Polyakov action for color images that minimizes the color manifold curvature.
			The color image curvature is computed by applying of the Laplace--Beltrami operator to the color image channels.
			When reduced to gray-scale images, while selecting appropriate scaling between space and color, the proposed model minimizes the Euler's elastica operating on the image level sets.
			Finding a minimizer for the proposed nonlinear geometric model is a challenge we address in this paper.
			Specifically, we present an operator-splitting method to minimize the proposed functional.
			The non-linearity is decoupled by introducing three vector-valued and matrix-valued variables.
			The problem is then converted into solving for the steady state of an associated initial-value problem.
			The initial-value problem is time-split into three fractional steps, such that each sub-problem has a closed form solution, or can be solved by fast algorithms.
			The efficiency and robustness of the proposed method are demonstrated by systematic numerical experiments.
		\end{abstract}
		
		\begin{keywords}
			Color image regularization, Operator-splitting, Polyakov action, Laplace--Beltrami, Euler's elastica
		\end{keywords}
		
		\begin{AMS}
			68U10, 94A08
		\end{AMS}
	


==> tmp_main_header.tex <==
	\title{A Color Elastica Model for Vector-Valued Image Regularization
		%\funding{Funding information goes here.}
	}
	
	\author{Hao Liu \thanks{School of Mathematics, Georgia Institute of Technology, Atlanta, GA 30332, USA. (\email{ hao.liu@math.gatech.edu}).}
		\and Xue-Cheng Tai \thanks{Department of Mathematics, Hong Kong Baptist University, Kowloon Tong, Hong Kong. (\email{ xuechengtai@hkbu.edu.hk}).}
		\and Ron Kimmel \thanks{Computer Science Department, Technion, Haifa, Israel. (\email{ ron@cs.technion.ac.il}).}
		\and Roland Glowinski \thanks{Department of Mathematics, University of Houston, Honston, TX 77204, USA. (\email{ roland@math.uh.edu}), and Department of Mathematics, Hong Kong Baptist University, Kowloon Tong, Hong Kong. }
	}
	
	% Custom SIAM macro to insert headers
	\headers{Color elastica model for vector-valued image regularization}{H. Liu, X.-C. Tai, R. Kimmel, and R. Glowinski}

